Intelligent Circuit Design and Implementation with Machine Learning

The stagnation of EDA technologies roots from insufficient knowledge reuse. In practice, very similar simulation or optimization results may need to be repeatedly constructed from scratch. This motivates my research on introducing more 'intelligence' to EDA with machine learning (ML), which explores complex correlations in design flows based on prior data. Besides design time, I also propose ML solutions to boost IC performance by assisting the circuit management at runtime. In this dissertation, I present multiple fast yet accurate ML models covering a wide range of chip design stages from the register-transfer level (RTL) to sign-off, solving primary chip-design problems about power, timing, interconnect, IR drop, routability, and design flow tuning. Targeting the RTL stage, I present APOLLO, a fully automated power modeling framework. It constructs an accurate per-cycle power model by extracting the most power-correlated signals. The model can be further implemented on chip for runtime power management with unprecedented low hardware costs. Targeting gate-level netlist, I present Net2 for early estimations on post-placement wirelength. It further enables more accurate timing analysis without actual physical design information. Targeting circuit layout, I present RouteNet for early routability prediction. As the first deep learning-based routability estimator, some feature-extraction and model-design principles proposed in it are widely adopted by later works. I also present PowerNet for fast IR drop estimation. It captures spatial and temporal information about power distribution with a customized CNN architecture. Last, besides targeting a single design step, I present FIST to efficiently tune design flow parameters during both logic synthesis and physical design.

==> txt/bob_macros.tex <==
%----  macros to save typing; added by hartley, 2002 ----
\newcommand{\fig}{\begin{figure}[htbp]\centering}
\newcommand{\pic}[1]{\includegraphics[width=#1]}
\newcommand{\efig}{\end{figure}} 
%\newcommand{\efig}{\end{figure} \clearpage}
% Use \clearpage to cure ``too many floats'' problem (1 fig. per page).
\newcommand{\fr}[1]{Figure \ref{fig:#1}}
\newcommand{\FR}[1]{Figure \ref{fig:#1}}
\newcommand{\er}[1]{equation \ref{eq:#1}}
\newcommand{\ER}[1]{Equation \ref{eq:#1}}
\newcommand{\eq}{\begin{equation}}
\newcommand{\eeq}{\end{equation}}
\newcommand{\eqa}{\begin{eqnarray}}
\newcommand{\eeqa}{\end{eqnarray}}
\newcommand{\etal}{\nobreak\mbox{\it et al.}}



\newcommand{\singlespacing}{%
  \let\CS=\small\renewcommand{\baselinestretch}{1.0}\CS}
\newcommand{\doublespacing}{%
  \let\CS=\small\renewcommand{\baselinestretch}{1.6}\CS}
\newcommand{\normalspacing}{\doublespacing}

%\newcommand{\singlespacingplus}{%
%  \let\CS=\@currsize\renewcommand{\baselinestretch}{1.25}\tiny\CS}
%\newcommand{\realdoublespacing}{%
%  \let\CS=\@currsize\renewcommand{\baselinestretch}{2}\tiny\CS}
%\newcommand{\footnotespacing}{\singlespacing}
%\newcommand{\changespacing}[2]{%
%  \renewcommand{#1}{%
%    \let\CS=\@currsize\renewcommand{\baselinestretch}{#2}\tiny\CS}%
%}
%\newcommand{\changenormalspacing}[1]{\renewcommand{\normalspacing}{#1}}




%---- units ----
\newcommand{\days}{\nobreak\mbox{$\;$days}}
\newcommand{\hrs}{\nobreak\mbox{$\;$hrs}}
\newcommand{\mins}{\nobreak\mbox{$\;$min}}
\newcommand{\s}{\nobreak\mbox{$\;$s}}
\newcommand{\ms}{\nobreak\mbox{$\;$ms}}
\newcommand{\us}{\nobreak\mbox{$\;\mu$s}}
\newcommand{\inch}{\nobreak\mbox{$\;$in}}
\newcommand{\meter}{\nobreak\mbox{$\;$m}}
\newcommand{\cm}{\nobreak\mbox{$\;$cm}}
\newcommand{\mm}{\nobreak\mbox{$\;$mm}}
\newcommand{\um}{\nobreak\mbox{$\;\mu$m}}
\newcommand{\nm}{\nobreak\mbox{$\;$nm}}
\newcommand{\cmpers}{\nobreak\mbox{$\;$cm\,s$^{-1}$}}
\newcommand{\mmpers}{\nobreak\mbox{$\;$mm\,s$^{-1}$}}
\newcommand{\umpers}{\nobreak\mbox{$\;\mu$m\,s$^{-1}$}}
\newcommand{\g}{\nobreak\mbox{$\;$g}}
\newcommand{\kg}{\nobreak\mbox{$\;$kg}}
\newcommand{\hz}{\nobreak\mbox{$\;$Hz}}
\newcommand{\mhz}{\nobreak\mbox{$\;$mHz}}
\newcommand{\uhz}{\nobreak\mbox{$\;\mu$Hz}}


%---- oft-used complicated symbols ----
\newcommand{\rms}{\nobreak\mbox{$\sigma_{rms}$}}
\newcommand{\sat}{\nobreak\mbox{$\sigma_{\textrm{sat}}$}}
\newcommand{\DG}{\nobreak\mbox{$\Delta G^2$}}
\newcommand{\DS}{\nobreak\mbox{$\Delta\sigma$}}
\newcommand{\DQ}{\nobreak\mbox{$\Delta\theta$}}
\newcommand{\DSDQ}{\nobreak\mbox{$\Delta\sigma/\Delta\theta$}}
\newcommand{\dq}{\nobreak\mbox{$d\theta$}}
\newcommand{\ds}{\nobreak\mbox{$d\sigma$}}
\newcommand{\dsdq}{\nobreak\mbox{$d\sigma/d\theta$}}
\newcommand{\YY}{$\curlyvee\curlywedge$}
\newcommand{\GG}{\nobreak\mbox{$G^2$}}


